Schematic Polymorphism in the Abella Proof Assistant

The Abella interactive theorem prover has proven to be an effective vehicle for reasoning about relational specifications. However, the system has a limitation that arises from the fact that it is based on a simply typed logic: formalizations that are identical except in the respect that they apply to different types have to be repeated at each type. We develop an approach that overcomes this limitation while preserving the logical underpinnings of the system. In this approach object constructors, formulas and other relevant logical notions are allowed to be parameterized by types, with the interpretation that they stand for the (infinite) collection of corresponding constructs that are obtained by instantiating the type parameters. The proof structures that we consider for formulas that are schematized in this fashion are limited to ones whose type instances are valid proofs in the simply typed logic. We develop schematic proof rules that ensure this property, a task that is complicated by the fact that type information influences the notion of unification that plays a key role in the logic. Our ideas, which have been implemented in an updated version of the system, accommodate schematic polymorphism both in the core logic of Abella and in the executable specification logic that it embeds.

==> conclusion.tex <==
\section{Concluding Remarks}
\label{sec:conclusion}

Our work has derived benefit from that on polymorphism for
higher-order logic programming
languages~\cite{nadathur92typesshort,hanus89iclpshort}, although there were
new complexities to consider both in embedding a specification
logic and in treating fixed-point definitions.
%
There are other systems such as Twelf~\cite{pfenning99cade}
and Beluga~\cite{pientka10ijcarshort} which provide reasoning capabilities
similar to \Abella and that also lack support of
polymorphism.
%
We believe that our ideas for schematic polymorphism can benefit
these systems as well and this is a topic worthy of exploration,
especially given their light-weight nature: our methods piggy-back
on existing mechanisms and should therefore be implementable with
limited additional effort.

%% We have presented an extension to a restricted view of the logic
%% underlying Abella with schematic polymorphism and demonstrated how it
%% enables induction and case analysis based reasoning about polymorphic
%% definitions in this logic and about polymorphic specifications in the
%% embedded logic of Horn clauses. Our discussion has covered the key
%% ideas for realizing schematic polymorphism, including parameterization
%% of fixed-point definitions over types at both the clause- and
%% block-level, parameterization of theorems over types, and proof
%% construction for such theorems using lifted proof rules whose
%% structures are insensitive to type information; the key to achieving
%% such type-insensitivity is the restriction of case analysis to
%% consider only unification problems with type-generic solutions.

%% By following the same ideas, we have extended the full logic
%% underlying Abella with schematic polymorphism. The extension enables
%% an embedding of the full HH specification logic in Abella and
%% induction and case analysis based reasoning about polymorphic programs
%% written in HH. We have applied it to implement and verify a compiler
%% for an extended version of PCF, and eliminated a significant amount of
%% redundancy in the libraries of specifications, theorems and proofs for
%% this project.
%% %
%% These developments are detailed in Wang's
%% Ph.D. thesis~\cite{wang16phd}.

%% The advantage of our schematic realization of polymorphism is that it
%% is a very light-weight way to introduce polymorphism to Abella. The
%% extended Abella system is based on the same underlying theory as the
%% original system, with only a thin layer of mechanisms for realizing
%% the schematization of the language and proofs. In fact, the whole
%% extension to Abella has been implemented in one month by one
%% person. The disadvantage is that theorems whose proofs specialize in
%% different ways under different type instantiations cannot be proved
%% using schematic polymorphism.

%% Finally, this work can be thought as an extension of the type system
%% for programming in higher-order logics~\cite{nadathur92types} to that
%% for reasoning about higher-order specifications with arguments
%% involving induction and case analysis. There are several other systems
%% with similar reasoning capability, such as Twelf~\cite{pfenning99cade}
%% and Beluga~\cite{pientka10ijcar}, that lack support of
%% polymorphism. We believe that the ideas for schematic polymorphism can
%% also be implemented in those systems and similar benefits can be
%% derived from the implementation.

%\vspace{-0.15cm}

